Exploring the Practicality of Generative Retrieval on Dynamic Corpora

Benchmarking the performance of information retrieval (IR) is mostly conducted with a fixed set of documents (static corpora). However, in realistic scenarios, this is rarely the case and the documents to be retrieved are constantly updated and added. In this paper, we focus on Generative Retrievals (GR), which apply autoregressive language models to IR problems, and explore their adaptability and robustness in dynamic scenarios. We also conduct an extensive evaluation of computational and memory efficiency, crucial factors for real-world deployment of IR systems handling vast and ever-changing document collections. Our results on the StreamingQA benchmark demonstrate that GR is more adaptable to evolving knowledge (4-11%), robust in learning knowledge with temporal information, and efficient in terms of inference FLOPs (x2), indexing time (x6), and storage footprint (x4) compared to Dual Encoders (DE), which are commonly used in retrieval systems. Our paper highlights the potential of GR for future use in practical IR systems within dynamic environments.

==> figs/adaptability.tex <==
\begin{figure}[ht!]
{
\centering
    \begin{minipage}[b]{0.50\textwidth}
    \includegraphics[width=\textwidth]{imgs/main_figure.png}
    \caption{}
    \end{minipage}
}
\label{fig:adaptability}
\end{figure}

==> figs/streamingir_illustration.tex <==
\begin{figure*}[t]
{
\includegraphics[width=0.99\linewidth]{imgs/streamingir_illustration.png}
}
\caption{Illustration on the temporal retrieval task considered in this work. The evidence articles are added in a streaming fashion, spanning from 2007 to 2020. In evaluation, questions are asked during the year 2020, where the query asks about either the most recent knowledge, and the past, static knowledge.}
\label{fig:streamingir_illustration}
\end{figure*}


==> tabs/2020_match.tex <==
\begin{table}[t!]
    \centering
    \tiny
    \setlength\tabcolsep{2.6pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{0.45\textwidth}{!}{
\begin{tabular}{cc|ccc}
\hline
 &  & \begin{tabular}[c]{@{}c@{}}Top-1 retrieved\\ passages of 2020\end{tabular} & \begin{tabular}[c]{@{}c@{}}Query \\ asked time\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gold\\ passage time\end{tabular} \\ \hline
\multirow{3}{*}{DE} & total & 56.09\% & 2020 & 2007-2020 \\
 & recent & 79.54\% & 2020 & 2020 \\
 & past & 27.23\% & 2020 & 2007-2019 \\ \hline
\multirow{3}{*}{GR} & total & 45.18\% & 2020 & 2007-2020 \\
 & recent & 65.67\% & 2020 & 2020 \\
 & past & 14.45\% & 2020 & 2007-2019 \\ \hline
\end{tabular}
}
    \caption{Percentage of top-1 retrieved passages with publication time of 2020. We can see that dual encoders tend to retrieve 2020 passages, almost twice as generative retrievers, even for the past subset. This means that 27\% of answers have no chance of being correct.}
    \label{tabs:2020_match}
\end{table}

==> tabs/efficiency.tex <==
\begin{table}[!]
    \centering
    \tiny
    \setlength\tabcolsep{3.2pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{0.35\textwidth}{!}{
\begin{tabular}{@{}cc|c|c@{}}
\toprule
 &  & bi(dpr) & gr(seal) \\ \midrule
model size &  & \textbf{110M} & 557M \\ \midrule
\multirow{2}{*}{indexing time} & full & 12hr & \textbf{0} \\
 & 2020 & 80min & \textbf{0} \\ \midrule
\begin{tabular}[c]{@{}c@{}}adaptation\\ (model update) time\end{tabular} & \begin{tabular}[c]{@{}c@{}}on \\ 2020\end{tabular} & \begin{tabular}[c]{@{}c@{}}approx.\\ 10hr\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}7.5hr \\ (1 epoch)\end{tabular}} \\ \midrule
\multirow{2}{*}{search time} & full & approx. 9hr & 85min \\
 & 2020 & approx. 2hr & -- \\ \midrule
\multirow{2}{*}{memory} & full & 150G & \textbf{32G} \\
 & 2020 & 18G & \textbf{4.2G} \\ \bottomrule
\end{tabular}
}
    \caption{Efficiency comparision with Bi-encoders and Generative ones. The search time of bi is based on the CPU version and it depends highly on the CPU resource. We assume a batch size of 128 per gpu for 4 gpus with beam size of 10 to measure GR decoding time.}
    \label{tabs:efficiency}
\end{table}

==> tabs/main_efficiency_table.tex <==
\begin{table*}[t!]
    \centering
    \tiny
    \setlength\tabcolsep{1.5pt}
    \renewcommand{\arraystretch}{1.45}
    % \setlength\tabcolsep{3pt}
    % \renewcommand{\arraystretch}{1.3}
    \resizebox{\textwidth}{!}{
    
\begin{tabular}{cl|cccccccc|cccccccccccc}
\hline
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{8}{c|}{Efficiency} &
  \multicolumn{12}{c}{Performance} \\ \hline
  & \multicolumn{1}{c|}{} &
  \multicolumn{2}{c|}{Memory} &
  \multicolumn{6}{c|}{Time (hours)} &
  \multicolumn{4}{c|}{Total (2007 -- 2020)} &
  \multicolumn{4}{c|}{Past (2007 -- 2019)} &
  \multicolumn{4}{c}{Recent (2020)} \\ \hline
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c}{Model} &
  \multicolumn{1}{c|}{Corpus} &
  \multicolumn{2}{c|}{End-to-end} &
  \multicolumn{2}{c|}{Train} &
  \multicolumn{2}{c|}{Eval} &
  \multicolumn{2}{c|}{Hits@} &
  \multicolumn{2}{c|}{Ans.Rec.@} &
  \multicolumn{2}{c|}{Hits@} &
  \multicolumn{2}{c|}{Ans.Rec.@} &
  \multicolumn{2}{c|}{Hits@} &
  \multicolumn{2}{c}{Ans.Rec.@} \\
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c}{\makecell{\#trained\\params}} &
  \multicolumn{1}{c|}{\makecell{index\\size}} &
  Train &
  \multicolumn{1}{c|}{Eval} &
  \makecell{pre-\\train} &
  \multicolumn{1}{c|}{\makecell{fine-\\tune}} &
  index &
  \multicolumn{1}{c|}{search} &
  5 &
  \multicolumn{1}{c|}{100} &
  5 &
  \multicolumn{1}{c|}{100} &
  5 &
  \multicolumn{1}{c|}{100} &
  5 &
  \multicolumn{1}{c|}{100} &
  5 &
  \multicolumn{1}{c|}{100} &
  5 &
  100 \\ \hline
 &
  \multicolumn{21}{c}{\textbf{supervised (pretrain + fine-tuned)}} \\ \hline
\multirow{3}{*}{bi} &
  \multicolumn{1}{l|}{2007--2019} &
  \multirow{3}{*}{110M} &
  \multicolumn{1}{c|}{18G} &
  47 &
  \multicolumn{1}{c|}{1.4} &
  45 &
  \multicolumn{1}{c|}{2} &
  1.3 &
  \textbf{0.1} &
  40.1 &
  \multicolumn{1}{c|}{67.4} &
  59.0 &
  \multicolumn{1}{c|}{83.7} &
  29.7 &
  \multicolumn{1}{c|}{57.2} &
  49.5 &
  \multicolumn{1}{c|}{80.7} &
  47.1 &
  \multicolumn{1}{c|}{74.2} &
  65.4 &
  85.6 \\
 &
  \multicolumn{1}{l|}{\quad + update} &
  &
  \multicolumn{1}{c|}{\multirow{2}{*}{150G}} &
  12 &
  \multicolumn{1}{c|}{\textcolor{red}{12.2}} &
  10 &
  \multicolumn{1}{c|}{2} &
  12 &
  0.2 &
  \textbf{43.0} &
  \multicolumn{1}{c|}{\textbf{71.1}} &
  \underline{61.5} &
  \multicolumn{1}{c|}{\textbf{85.4}} &
  30.7 &
  \multicolumn{1}{c|}{58.7} &
  49.6 &
  \multicolumn{1}{c|}{81.9} &
  \underline{51.2} &
  \multicolumn{1}{c|}{\underline{79.3}} &
  \underline{69.4} &
  \underline{87.7} \\
 &
  \multicolumn{1}{l|}{\quad + 2020 Q} &
   &
  \multicolumn{1}{c|}{} &
  15 &
  \multicolumn{1}{c|}{\textcolor{red}{12.2}} &
  10 &
  \multicolumn{1}{c|}{5} &
  12&
  0.2 &
  \underline{42.3} &
  \multicolumn{1}{c|}{68.1} &
  59.4 &
  \multicolumn{1}{c|}{82.4} &
  20.9 &
  \multicolumn{1}{c|}{45.0} &
  38.7 &
  \multicolumn{1}{c|}{72.5} &
  \textbf{56.6} &
  \multicolumn{1}{c|}{\textbf{83.5}} &
  \textbf{73.1} &
  \textbf{89.0} \\ \hdashline[2pt/1pt]
\multirow{2}{*}{gr} &
  \multicolumn{1}{l|}{2007--2019} &
  557M &
  \multicolumn{1}{c|}{\textbf{4.2G}} &
  21.7 &
  \multicolumn{1}{c|}{\textbf{0.8}} &
  21* &
  \multicolumn{1}{c|}{\textbf{0.7}} &
  \textbf{0} &
  0.8 &
  33.2 &
  \multicolumn{1}{c|}{59.5} &
  55.7 &
  \multicolumn{1}{c|}{81.2} &
  \underline{32.8} &
  \multicolumn{1}{c|}{\underline{60.6}} &
  \underline{56.8} &
  \multicolumn{1}{c|}{\underline{82.8}} &
  33.5 &
  \multicolumn{1}{c|}{58.9} &
  54.9 &
  80.2 \\
  &
  \multicolumn{1}{l|}{\quad + up. + 2020 Q} &
  \textbf{3M} &
  \multicolumn{1}{c|}{32G} &
  \textbf{8.5} &
  \multicolumn{1}{c|}{\textbf{0.8}} &
  \textbf{7.5} &
  \multicolumn{1}{c|}{1} &
  \textbf{0} &
  0.8 &
  41.6 &
  \multicolumn{1}{c|}{\underline{68.3}} &
  \textbf{62.9} &
  \multicolumn{1}{c|}{\underline{85.2}} &
  \textbf{38.3} &
  \multicolumn{1}{c|}{\textbf{65.0}} &
  \textbf{60.0} &
  \multicolumn{1}{c|}{\textbf{84.1}} &
  43.8 &
  \multicolumn{1}{c|}{70.6} &
  64.9 &
  85.9 \\ \hline
\end{tabular}

}
    \caption{Performance and efficiency analysis of Bi and GR variants, evaluated on the 5000 past and recent subsets. All environments consider one A100 80GB GPU except * (evaluated on different GPUs).
    % The best and the second best performance are highlighted with bold and underline, respectively.
    % For efficiency, faster \& smaller is better. For performance, higher score is better.
    While updated bi-encoder and generative retrieval perform competitively, we observe that updating bi-encoder is inefficient overall, in particular with an excessive evaluation time cost of \textcolor{red}{12.2 hours} caused by indexing opposed to \textbf{0.8 hours} of generative retrieval.}
    \label{tabs:main_efficiency_table}
\end{table*}

==> tabs/main_table.tex <==
\begin{table*}[t]
    \centering
    %\tiny \hdashline[2pt/2pt]
    %\setlength\tabcolsep{1.5pt}
    \renewcommand{\arraystretch}{1.45}
    \resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccccc}
\hline
\multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Performance (hits@5)} & \multicolumn{5}{c}{Efficiency} \\ \hline
\multicolumn{1}{c|}{model name} & total & past & recent & \begin{tabular}[c]{@{}c@{}}trainable\\ param.\end{tabular} & \begin{tabular}[c]{@{}c@{}}time\\ from scratch\end{tabular} & \begin{tabular}[c]{@{}c@{}}training\\ flops\end{tabular} & \begin{tabular}[c]{@{}c@{}}index + \\ search time\end{tabular} & \begin{tabular}[c]{@{}c@{}}index \\ memory\end{tabular} \\ \hline
DE-past & 26.32\% & 18.20\% & 34.43\% & 110M & 43.7 & 2.55E+19 & 10.4 & 132G \\
DE & 39.81\% & 29.75\% & 49.87\% & 110M & 52.5 & 6.09E+18 & 12.3 & 150G \\
DE + 2020 Q & 35.29\% & 20.55\% & \textbf{50.03\%} & 110M & 54.0 & 6.35E+18 & 12.3 & 150G \\ \hdashline[2pt/2pt]
GR-past & 33.15\% & 32.80\% & 33.50\% & 557M & 25.4 & 2.31E+19 & 3.1 & 28G \\
GR-full & 31.60\% & 31.50\% & 31.70\% & 557M & 34.4 & 3.60E+19 & \textbf{4.5} & \textbf{32G} \\
GR-convent.LoRA & 31.69\% & 32.00\% & 31.37\% & \textbf{2.4M} & \textbf{28.9} & \textbf{3.60E+17} & \textbf{4.5} & \textbf{32G} \\
DynamicGR & 38.08\% & 37.25\% & 38.90\% & 3.1M & 32.8 & 3.65E+17 & \textbf{4.5} & \textbf{32G} \\
DynamicGR + 2020 Q & \textbf{41.01\%} & \textbf{38.25\%} & 43.77\% & 3.1M & 33.6 & 7.11E+17 & \textbf{4.5} & \textbf{32G} \\ \hline
\end{tabular}
}
    \caption{Efficiency and performance on dual encoder and generative retrieval variants. For the model name description, please see Section \ref{sec:model_name}. We evaluate retrieval performance in three ways: (1) past knowledge retention in the 'past' category, (2) updated knowledge acquisition in the 'recent' category, and (3) a comprehensive assessment of the 'past + recent' subset, which represents the unweighted average in the 'total' category. In addition, we present the core components of our evaluation, along with three primary axes. The first axis distinguishes between before and after the update. The second axis focuses on pre-training methods specific to GR (GR-full, GR-convent.LoRA, and DynamicGR). The third axis examines the integration of additional supervised data from the updated corpus (DE + 2020 Q and DynamicGR + 2020Q). We highlight the most outstanding results in \textbf{bold} during the updates. Full stats including answer recall are at appendix Table \ref{tabs:appendix_hits_performance} and \ref{tabs:appendix_answer_recall_performance}.}
    \label{tabs:main_table}
\end{table*}






    
    
    %We can observe that na\"ive fine-tuning the generative retrieval model fails on recent eval sets, and employing DynamicGR is the most effective compared with the corresponding dual model. We can also see that generative retrievers are more memory and parameter efficient for update scenarios. Full stats including answer recall are at appendix Table \ref{tabs:appendix_hits_performance} and \ref{tabs:appendix_answer_recall_performance}.}
    \label{tabs:main_table}
%\end{table*}

==> tabs/main_table_deprecated.tex <==
\begin{table*}[t]
    \centering
    \tiny
    \setlength\tabcolsep{3.2pt}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{0.9\textwidth}{!}{
    
\begin{tabular}{cccccccccc}
                            & \multicolumn{1}{c|}{}          & \multicolumn{4}{c|}{hits@N}                                                                    & \multicolumn{4}{c}{answer recall@N}                                       \\ \cline{3-10} 
                            & \multicolumn{1}{c|}{}          & 5                & 10               & 50               & \multicolumn{1}{c|}{100}              & 5                & 10               & 50               & 100              \\ \hline
\multicolumn{10}{c}{zero-shot}                                                                                                                                                                                                            \\ \hline
traditional                 & \multicolumn{1}{c|}{bm25}     & 48.64\%          & 55.60\%          & 70.04\%          & \multicolumn{1}{c|}{74.72\%}          & 67.28\%          & 73.64\%          & 84.60\%          & 86.76\%          \\
\multirow{3}{*}{bi}         & \multicolumn{1}{c|}{dpr-kilt}  & 11.26\%          & 14.34\%          & 23.92\%          & \multicolumn{1}{c|}{27.74\%}          & 32.54\%          & 40.36\%          & 56.70\%          & 61.96\%          \\
                            & \multicolumn{1}{c|}{spider}    & 16.94\%          & 22.56\%          & 37.10\%          & \multicolumn{1}{c|}{42.46\%}          & 26.64\%          & 35.48\%          & 55.76\%          & 61.68\%          \\
                            & \multicolumn{1}{c|}{spider-nq} & 14.14\%          & 18.64\%          & 30.02\%          & \multicolumn{1}{c|}{34.06\%}          & 31.88\%          & 40.42\%          & 57.10\%          & 62.12\%          \\
gr                          & \multicolumn{1}{c|}{seal-kilt} & \textbf{20.76\%} & \textbf{26.66\%} & \textbf{42.10\%} & \multicolumn{1}{c|}{\textbf{49.64\%}} & \textbf{45.24\%} & \textbf{54.02\%} & \textbf{72.52\%} & \textbf{77.68\%} \\ \hline
\multicolumn{10}{c}{unsupervised (with only pretraining)}                                                                                                                                                                                 \\ \hline
\multirow{2}{*}{$\sim$2019} & \multicolumn{1}{c|}{bi}        & 20.50\%          & 25.32\%          & 38.22\%          & \multicolumn{1}{c|}{41.50\%}          & 37.42\%          & 44.84\%          & 61.62\%          & 66.00\%          \\
                            & \multicolumn{1}{c|}{gr}        & 34.46\%           & 38.92\%           & 49.16\%           & \multicolumn{1}{c|}{52.82\%}           & 47.22\%           & 54.46\%           & 68.84\%           & 73.30\%           \\
\multirow{2}{*}{$\sim$2020} & \multicolumn{1}{c|}{bi}        & 19.45\%          & 24.30\%          & 37.45\%          & \multicolumn{1}{c|}{41.81\%}          & 39.25\%          & 47.78\%          & 65.60\%          & 70.11\%          \\
                            & \multicolumn{1}{c|}{gr}        & \textbf{34.34\%} & \textbf{38.86\%} & \textbf{49.04\%} & \multicolumn{1}{c|}{\textbf{52.76\%}} & \textbf{47.18\%} & \textbf{54.46\%} & \textbf{68.60\%} & \textbf{73.12\%} \\ \hline
\multicolumn{10}{c}{supervised (fine-tuned)}                                                                                                                                                                                              \\ \hline
\multirow{2}{*}{$\sim$2019} & \multicolumn{1}{c|}{bi}        & 40.10\%          & 47.56\%          & 63.32\%          & \multicolumn{1}{c|}{67.36\%}          & 59.04\%          & 67.46\%          & 81.02\%          & 83.66\%          \\
                            & \multicolumn{1}{c|}{gr}        & 33.20\%          & 39.78\%          & 54.06\%          & \multicolumn{1}{c|}{59.54\%}          & 55.66\%          & 63.52\%          & 77.30\%          & 81.24\%          \\
\multirow{2}{*}{$\sim$2020} & \multicolumn{1}{c|}{bi}        & \textbf{42.96\%} & \textbf{50.86\%} & \textbf{66.76\%} & \multicolumn{1}{c|}{\textbf{71.06\%}} & 61.46\%          & 69.80\%          & \textbf{82.96\%} & 85.38\%          \\
                            & \multicolumn{1}{c|}{gr}        & 41.54\%          & 48.00\%          & 62.70\%          & \multicolumn{1}{c|}{68.54\%}          & \textbf{62.46\%} & \textbf{69.90\%} & 81.92\%          & \textbf{85.56\%} \\ \hline
\end{tabular}
}
    \caption{Hits and Answer recall (\%) for the passage-leve retrieval task on streamingqa. \textbf{Bold} and \underline{underline} indicates the best and second model respectively. TBU.}
    \label{tabs:main_table}
\end{table*}

==> tabs/main_table_depreceated.tex <==
\begin{table*}[t]
    \centering
    \tiny
    \setlength\tabcolsep{3.2pt}
    \newcolumntype{?}{!{\vrule width 1pt}}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\textwidth}{!}{

\begin{tabular}{ccc?cccc?cccc?ccccc}
%\cline{4-16}
\textbf{} &
   &
   &
  \multicolumn{4}{c?}{zero-shot} &
  \multicolumn{4}{c?}{unsupervised (only pretraining)} &
  \multicolumn{5}{c}{supervised (pretrain + fine-tuned)} \\ \cline{4-16} 
 &
   &
   &
  \multicolumn{3}{c}{bi} &
  gr &
  \multicolumn{2}{c}{$\sim$2019} &
  \multicolumn{2}{c?}{$\sim$2020} &
  \multicolumn{2}{c}{$\sim$2019} &
  \multicolumn{3}{c}{GR variants, after update} \\ \cline{4-16} 
 &
   &
   &
  \begin{tabular}[c]{@{}c@{}}dpr-\\ multi\end{tabular} &
  spider &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}spider\\ +nq\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}seal\\ -kilt\end{tabular} &
  bi &
  \multicolumn{1}{c|}{gr} &
  bi &
  gr &
  bi &
  \multicolumn{1}{c|}{gr} &
  \begin{tabular}[c]{@{}c@{}}full fine-\\ tuning\end{tabular} &
  \multicolumn{1}{l}{LoRA} &
  \begin{tabular}[c]{@{}c@{}}LoRA +\\ 2020 query\end{tabular} \\ \Xhline{2\arrayrulewidth}
\multirow{8}{*}{TOTAL} &
  \multirow{4}{*}{hits@N} &
  5 &
  11.26 &
  16.94 &
  \multicolumn{1}{c|}{14.14} &
  20.76 &
  20.50 &
  \multicolumn{1}{c|}{34.46} &
  19.45 &
  34.34 &
  40.10 &
  \multicolumn{1}{c|}{33.20} &
  31.68 &
  38.24 &
  \textbf{41.56} \\
 &
   &
  10 &
  14.34 &
  22.56 &
  \multicolumn{1}{c|}{18.64} &
  26.66 &
  25.32 &
  \multicolumn{1}{c|}{38.92} &
  24.30 &
  38.86 &
  47.56 &
  \multicolumn{1}{c|}{39.78} &
  37.13 &
  44.12 &
  \textbf{48.52} \\
 &
   &
  50 &
  23.92 &
  37.10 &
  \multicolumn{1}{c|}{30.02} &
  42.10 &
  38.22 &
  \multicolumn{1}{c|}{49.16} &
  37.45 &
  49.04 &
  \textbf{63.32} &
  \multicolumn{1}{c|}{54.06} &
  51.06 &
  58.54 &
  63.44 \\
 &
   &
  100 &
  27.74 &
  42.46 &
  \multicolumn{1}{c|}{34.06} &
  49.64 &
  41.50 &
  \multicolumn{1}{c|}{52.82} &
  41.81 &
  52.76 &
  67.36 &
  \multicolumn{1}{c|}{59.54} &
  56.12 &
  64.44 &
  \textbf{68.34} \\ \cline{2-16} 
 &
  \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}answer \\ recall@N\end{tabular}} &
  5 &
  32.54 &
  26.64 &
  \multicolumn{1}{c|}{31.88} &
  45.24 &
  37.42 &
  \multicolumn{1}{c|}{47.22} &
  39.25 &
  47.18 &
  59.04 &
  \multicolumn{1}{c|}{55.66} &
  51.70 &
  59.66 &
  \textbf{62.94} \\
 &
   &
  10 &
  40.36 &
  35.48 &
  \multicolumn{1}{c|}{40.42} &
  54.02 &
  44.84 &
  \multicolumn{1}{c|}{54.46} &
  47.78 &
  54.46 &
  67.46 &
  \multicolumn{1}{c|}{63.52} &
  59.52 &
  67.36 &
  \textbf{70.68} \\
 &
   &
  50 &
  56.70 &
  55.76 &
  \multicolumn{1}{c|}{57.10} &
  72.52 &
  61.62 &
  \multicolumn{1}{c|}{68.84} &
  65.60 &
  68.60 &
  81.02 &
  \multicolumn{1}{c|}{77.30} &
  72.56 &
  80.30 &
  \textbf{81.92} \\
 &
   &
  100 &
  61.96 &
  61.68 &
  \multicolumn{1}{c|}{62.12} &
  77.68 &
  66.00 &
  \multicolumn{1}{c|}{73.30} &
  70.11 &
  73.12 &
  83.66 &
  \multicolumn{1}{c|}{81.24} &
  76.06 &
  83.88 &
  \textbf{85.20} \\ \Xhline{2\arrayrulewidth}
\multirow{8}{*}{PAST} &
  \multirow{4}{*}{hits@N} &
  5 &
  9.00 &
  12.65 &
  \multicolumn{1}{c|}{8.95} &
  19.80 &
  6.65 &
  \multicolumn{1}{c|}{32.70} &
  12.30 &
  32.65 &
  29.65 &
  \multicolumn{1}{c|}{32.75} &
  29.90 &
  37.25 &
  \textbf{38.25} \\
 &
   &
  10 &
  11.95 &
  17.05 &
  \multicolumn{1}{c|}{11.95} &
  25.75 &
  8.45 &
  \multicolumn{1}{c|}{37.45} &
  15.77 &
  37.50 &
  35.75 &
  \multicolumn{1}{c|}{38.90} &
  35.75 &
  43.15 &
  \textbf{45.30} \\
 &
   &
  50 &
  20.10 &
  28.75 &
  \multicolumn{1}{c|}{19.15} &
  41.70 &
  15.95 &
  \multicolumn{1}{c|}{48.85} &
  26.49 &
  48.70 &
  51.85 &
  \multicolumn{1}{c|}{54.50} &
  49.55 &
  58.25 &
  \textbf{60.20} \\
 &
   &
  100 &
  23.35 &
  33.45 &
  \multicolumn{1}{c|}{22.25} &
  49.90 &
  17.55 &
  \multicolumn{1}{c|}{52.40} &
  30.44 &
  52.20 &
  57.15 &
  \multicolumn{1}{c|}{60.55} &
  54.75 &
  64.40 &
  \textbf{65.00} \\ \cline{2-16} 
 &
  \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}answer \\ recall@N\end{tabular}} &
  5 &
  28.50 &
  21.00 &
  \multicolumn{1}{c|}{24.50} &
  45.10 &
  20.00 &
  \multicolumn{1}{c|}{45.25} &
  30.08 &
  45.15 &
  49.45 &
  \multicolumn{1}{c|}{56.80} &
  50.85 &
  59.20 &
  \textbf{59.95} \\
 &
   &
  10 &
  35.80 &
  29.05 &
  \multicolumn{1}{c|}{31.70} &
  54.40 &
  26.35 &
  \multicolumn{1}{c|}{52.50} &
  38.60 &
  52.75 &
  58.95 &
  \multicolumn{1}{c|}{64.45} &
  58.95 &
  67.65 &
  \textbf{68.10} \\
 &
   &
  50 &
  53.55 &
  49.70 &
  \multicolumn{1}{c|}{47.70} &
  74.10 &
  44.75 &
  \multicolumn{1}{c|}{68.75} &
  57.83 &
  68.55 &
  76.50 &
  \multicolumn{1}{c|}{78.95} &
  72.20 &
  81.30 &
  \textbf{80.30} \\
 &
   &
  100 &
  58.90 &
  56.40 &
  \multicolumn{1}{c|}{53.30} &
  79.50 &
  50.30 &
  \multicolumn{1}{c|}{73.30} &
  63.31 &
  73.00 &
  80.70 &
  \multicolumn{1}{c|}{82.75} &
  76.05 &
  85.15 &
  \textbf{84.10} \\ \Xhline{2\arrayrulewidth}
\multirow{8}{*}{RECENT} &
  \multirow{4}{*}{hits@N} &
  5 &
  12.77 &
  19.80 &
  \multicolumn{1}{c|}{17.60} &
  21.40 &
  29.73 &
  \multicolumn{1}{c|}{35.63} &
  24.66 &
  35.47 &
  \textbf{47.07} &
  \multicolumn{1}{c|}{33.50} &
  32.87 &
  38.90 &
  43.77 \\
 &
   &
  10 &
  15.93 &
  26.23 &
  \multicolumn{1}{c|}{23.10} &
  27.27 &
  36.57 &
  \multicolumn{1}{c|}{39.90} &
  30.51 &
  39.77 &
  \textbf{55.43} &
  \multicolumn{1}{c|}{40.37} &
  38.05 &
  44.77 &
  50.67 \\
 &
   &
  50 &
  26.47 &
  42.67 &
  \multicolumn{1}{c|}{37.27} &
  42.37 &
  53.07 &
  \multicolumn{1}{c|}{49.37} &
  45.33 &
  49.27 &
  \textbf{70.97} &
  \multicolumn{1}{c|}{53.77} &
  52.07 &
  58.73 &
  65.60 \\
 &
   &
  100 &
  30.67 &
  48.47 &
  \multicolumn{1}{c|}{41.93} &
  49.47 &
  57.47 &
  \multicolumn{1}{c|}{53.10} &
  49.99 &
  53.13 &
  \textbf{74.17} &
  \multicolumn{1}{c|}{58.87} &
  57.03 &
  64.47 &
  70.57 \\ \cline{2-16} 
 &
  \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}answer \\ recall@N\end{tabular}} &
  5 &
  35.23 &
  30.40 &
  \multicolumn{1}{c|}{36.80} &
  45.33 &
  49.03 &
  \multicolumn{1}{c|}{48.53} &
  46.20 &
  48.53 &
  \textbf{65.43} &
  \multicolumn{1}{c|}{54.90} &
  52.27 &
  59.97 &
  64.93 \\
 &
   &
  10 &
  43.40 &
  39.77 &
  \multicolumn{1}{c|}{46.23} &
  53.77 &
  57.17 &
  \multicolumn{1}{c|}{55.77} &
  54.79 &
  55.60 &
  \textbf{73.13} &
  \multicolumn{1}{c|}{62.90} &
  59.90 &
  67.17 &
  72.40 \\
 &
   &
  50 &
  58.80 &
  59.80 &
  \multicolumn{1}{c|}{63.37} &
  71.47 &
  72.87 &
  \multicolumn{1}{c|}{68.90} &
  71.60 &
  68.64 &
  \textbf{84.03} &
  \multicolumn{1}{c|}{76.20} &
  72.80 &
  79.63 &
  83.00 \\
 &
   &
  100 &
  64.00 &
  65.20 &
  \multicolumn{1}{c|}{68.00} &
  76.46 &
  76.47 &
  \multicolumn{1}{c|}{73.30} &
  75.33 &
  73.20 &
  85.63 &
  \multicolumn{1}{c|}{80.23} &
  76.07 &
  83.03 &
  \textbf{85.93} \\ \Xhline{2\arrayrulewidth}
\end{tabular}

}
    \caption{Hits and Answer recall (\%) for the passage-level retrieval task on streamingqa. \textbf{Bold} indicates the best model. bi represents the dual-encoder variant based on the DPR archiecture, and gr refers to SEAL.}
    \label{tabs:main_table_deprecated}
\end{table*}


% \Xhline{2\arrayrulewidth}
% \newcolumntype{?}{!{\vrule width 1pt}}

==> tabs/main_table_transposed_deprecated.tex <==
\begin{table*}[t]
    \centering
    \tiny
    \setlength\tabcolsep{1.5pt}
    \renewcommand{\arraystretch}{1.45}
    \resizebox{\textwidth}{!}{

\begin{tabular}{clcccccccccccccccccccccccc}
\hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{8}{c|}{Total (2007 -- 2020)} &
  \multicolumn{8}{c|}{Past (2007 -- 2019)} &
  \multicolumn{8}{c}{Recent (2020)} \\ \hline
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{4}{c|}{Hits@N} &
  \multicolumn{4}{c|}{Answer Recall@N} &
  \multicolumn{4}{c|}{Hits@N} &
  \multicolumn{4}{c|}{Answer Recall@N} &
  \multicolumn{4}{c|}{Hits@N} &
  \multicolumn{4}{c}{Answer Recall@N} \\
 &
  \multicolumn{1}{l|}{} &
  5 &
  10 &
  50 &
  \multicolumn{1}{c|}{100} &
  5 &
  10 &
  50 &
  \multicolumn{1}{c|}{100} &
  5 &
  10 &
  50 &
  \multicolumn{1}{c|}{100} &
  5 &
  10 &
  50 &
  \multicolumn{1}{c|}{100} &
  5 &
  10 &
  50 &
  \multicolumn{1}{c|}{100} &
  5 &
  10 &
  50 &
  100 \\ \hline
\multicolumn{26}{c}{\textbf{only fine-tuning without pretraining}} \\ \hline
bi &
  \multicolumn{1}{c|}{ft} &
  24.8 &
  30.5 &
  44.5 &
  \multicolumn{1}{c|}{49.1} &
  44.6 &
  53.3 &
  69.7 &
  \multicolumn{1}{c|}{73.9} &
  17.9 &
  22.1 &
  34.5 &
  \multicolumn{1}{c|}{38.6} &
  35.7 &
  44.6 &
  63.0 &
  \multicolumn{1}{c|}{68.3} &
  29.4 &
  36.1 &
  51.2 &
  \multicolumn{1}{c|}{56.1} &
  50.5 &
  59.1 &
  74.1 &
  77.7 \\ \hdashline[2pt/1pt]
gr &
  \multicolumn{1}{c|}{ft} &
  13.8 &
  16.6 &
  22.8 &
  \multicolumn{1}{c|}{25.1} &
  37.4 &
  43.8 &
  55.8 &
  \multicolumn{1}{c|}{60.0} &
  32.4 &
  39.1 &
  54.1 &
  \multicolumn{1}{c|}{60.0} &
  55.6 &
  63.1 &
  77.1 &
  \multicolumn{1}{c|}{79.9} &
  \textcolor{red}{1.4} &
  \textcolor{red}{1.6} &
  \textcolor{red}{2.0} &
  \multicolumn{1}{c|}{\textcolor{red}{2.1}} &
  25.3 &
  30.9 &
  41.7 &
  46.7 \\ \hline
\multicolumn{26}{c}{\textbf{unsupervised (only pretraining)}} \\ \hline
\multirow{2}{*}{bi} &
  \multicolumn{1}{c|}{2007 -- 2019} &
  20.5 &
  25.3 &
  38.2 &
  \multicolumn{1}{c|}{41.5} &
  37.4 &
  44.8 &
  61.6 &
  \multicolumn{1}{c|}{66.0} &
  6.7 &
  8.5 &
  16.0 &
  \multicolumn{1}{c|}{17.6} &
  20.0 &
  26.4 &
  44.8 &
  \multicolumn{1}{c|}{50.3} &
  29.7 &
  36.6 &
  53.1 &
  \multicolumn{1}{c|}{57.5} &
  49.0 &
  57.2 &
  72.9 &
  76.5 \\
 &
  \multicolumn{1}{c|}{+ 2020} &
  19.5 &
  24.3 &
  37.5 &
  \multicolumn{1}{c|}{41.8} &
  39.2 &
  47.8 &
  65.6 &
  \multicolumn{1}{c|}{70.1} &
  12.3 &
  15.8 &
  26.5 &
  \multicolumn{1}{c|}{30.4} &
  30.1 &
  38.6 &
  57.8 &
  \multicolumn{1}{c|}{63.3} &
  24.7 &
  30.5 &
  45.3 &
  \multicolumn{1}{c|}{50.0} &
  46.2 &
  54.8 &
  71.6 &
  75.3 \\ \hdashline[2pt/1pt]
\multirow{2}{*}{gr} &
  \multicolumn{1}{c|}{2007 -- 2019} &
  34.5 &
  38.9 &
  49.2 &
  \multicolumn{1}{c|}{52.8} &
  47.2 &
  54.5 &
  68.8 &
  \multicolumn{1}{c|}{73.3} &
  32.7 &
  37.5 &
  48.9 &
  \multicolumn{1}{c|}{52.4} &
  45.3 &
  52.5 &
  68.8 &
  \multicolumn{1}{c|}{73.3} &
  35.6 &
  39.9 &
  49.4 &
  \multicolumn{1}{c|}{53.1} &
  48.5 &
  55.8 &
  68.9 &
  73.3 \\
 &
  \multicolumn{1}{c|}{+ 2020} &
  34.3 &
  38.9 &
  49.0 &
  \multicolumn{1}{c|}{52.8} &
  47.2 &
  54.5 &
  68.6 &
  \multicolumn{1}{c|}{73.1} &
  32.7 &
  37.5 &
  48.7 &
  \multicolumn{1}{c|}{52.2} &
  45.2 &
  52.8 &
  68.6 &
  \multicolumn{1}{c|}{73.0} &
  35.5 &
  39.8 &
  49.3 &
  \multicolumn{1}{c|}{53.1} &
  48.5 &
  55.6 &
  68.6 &
  73.2 \\ \hline
\multicolumn{26}{c}{\textbf{supervised (pretrain + fine-tuned)}} \\ \hline
bi &
  \multicolumn{1}{l|}{2007 -- 2019 + ft} &
  40.1 &
  47.6 &
  63.3 &
  \multicolumn{1}{c|}{67.4} &
  59.0 &
  67.5 &
  81.0 &
  \multicolumn{1}{c|}{83.7} &
  29.7 &
  35.8 &
  51.9 &
  \multicolumn{1}{c|}{57.2} &
  49.5 &
  59.0 &
  76.5 &
  \multicolumn{1}{c|}{80.7} &
  \textbf{47.1} &
  \textbf{55.4} &
  \textbf{71.0} &
  \multicolumn{1}{c|}{\textbf{74.2}} &
  \textbf{65.4} &
  \textbf{73.1} &
  \textbf{84.0} &
  85.6 \\ \hdashline[2pt/1pt]
\multirow{1}{*}{gr} &
  \multicolumn{1}{l|}{2007 -- 2019} &
  33.2 &
  39.8 &
  54.1 &
  \multicolumn{1}{c|}{59.5} &
  55.7 &
  63.5 &
  77.3 &
  \multicolumn{1}{c|}{81.2} &
  32.8 &
  38.9 &
  54.5 &
  \multicolumn{1}{c|}{60.6} &
  56.8 &
  64.5 &
  79.0 &
  \multicolumn{1}{c|}{82.8} &
  33.5 &
  40.4 &
  53.8 &
  \multicolumn{1}{c|}{58.9} &
  54.9 &
  62.9 &
  76.2 &
  80.2 \\
 &
  \multicolumn{1}{l|}{+ full pretrain + ft} &
  31.7 &
  37.1 &
  51.1 &
  \multicolumn{1}{c|}{56.1} &
  51.7 &
  59.5 &
  72.6 &
  \multicolumn{1}{c|}{76.1} &
  29.9 &
  35.8 &
  49.6 &
  \multicolumn{1}{c|}{54.8} &
  50.9 &
  59.0 &
  72.2 &
  \multicolumn{1}{c|}{76.1} &
  32.9 &
  38.1 &
  52.1 &
  \multicolumn{1}{c|}{57.0} &
  52.3 &
  59.9 &
  72.8 &
  76.1 \\
 &
  \multicolumn{1}{l|}{+ LoRA (att.) + ft} &
  33.3 &
  39.7 &
  54.0 &
  \multicolumn{1}{c|}{59.5} &
  54.7 &
  62.8 &
  75.7 &
  \multicolumn{1}{c|}{79.3} &
  32.6 &
  39.2 &
  54.2 &
  \multicolumn{1}{c|}{60.4} &
  55.4 &
  64.1 &
  76.7 &
  \multicolumn{1}{c|}{80.6} &
  33.7 &
  40.1 &
  53.9 &
  \multicolumn{1}{c|}{58.9} &
  54.2 &
  61.9 &
  75.0 &
  78.4 \\
 &
  \multicolumn{1}{l|}{+ LoRA (exp.) + ft} &
  38.2 &
  44.1 &
  58.5 &
  \multicolumn{1}{c|}{64.4} &
  59.7 &
  67.4 &
  80.3 &
  \multicolumn{1}{c|}{83.9} &
  37.3 &
  43.2 &
  58.3 &
  \multicolumn{1}{c|}{64.4} &
  59.2 &
  67.7 &
  \textbf{81.3} &
  \multicolumn{1}{c|}{\textbf{85.2}} &
  38.9 &
  44.8 &
  58.7 &
  \multicolumn{1}{c|}{64.5} &
  60.0 &
  67.2 &
  79.6 &
  83.0 \\
 &
  \multicolumn{1}{l|}{\quad \quad + ft w/ 2020 Q} &
  \textbf{41.6} &
  \textbf{48.5} &
  \textbf{63.4} &
  \multicolumn{1}{c|}{\textbf{68.3}} &
  \textbf{62.9} &
  \textbf{70.7} &
  \textbf{81.9} &
  \multicolumn{1}{c|}{\textbf{85.2}} &
  \textbf{38.3} &
  \textbf{45.3} &
  \textbf{60.2} &
  \multicolumn{1}{c|}{\textbf{65.0}} &
  \textbf{60.0} &
  \textbf{68.1} &
  80.3 &
  \multicolumn{1}{c|}{84.1} &
  43.8 &
  50.7 &
  65.6 &
  \multicolumn{1}{c|}{70.6} &
  64.9 &
  72.4 &
  83.0 &
  \textbf{85.9} \\ \hline
\end{tabular}

}
    \caption{Hits and Answer recall (\%) for the passage-level retrieval task on \textsc{StreamingIR}. \textbf{Bold} indicates the best score. ft means fine-tuned, and LoRA (att.) and LoRA (exp.) means LoRA attached only on attention, and LoRA expanded to fully connected layers, respectively. We can see that na\"ive fine-tuning the GR (Generative Retrieval) model \textcolor{red}{fail} on recent eval sets, and that GR benefits a lot from pre-training. Among the pre-training methods, using LoRA was the most effective with respect to the corresponding bi model. }
    \label{tabs:main_table_transp_deprecated}
\end{table*}

==> tabs/no_train_update.tex <==
%\usepackage[symbol]{footmisc}
%\newcounter{mpFootnoteValueSaver}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\begin{table*}[t!]
%newcounter{mpFootnoteValueSaver}
%setcounter{mpFootnoteValueSaver}{\value{footnote}}
\centering
\fontsize{9}{13}\selectfont
\begin{threeparttable}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccc}
        \toprule
             & \multicolumn{3}{c}{Performance $(hit@5)$} & \multicolumn{4}{c}{Efficiency} \\
                \cmidrule(lr){2-4} \cmidrule(lr){5-8}  
            \makecell{Evaluation} & \makecell{$Q_{\textit{total}}$} & \makecell{$Q_{\textit{initial}}$} & \makecell{$Q_{\textit{new}}$} & \makecell{Inference Flops} & \makecell{Indexing Time} & \makecell{Inference Latency \\ ($T_{\textit{online}}$ / $T_{\textit{offline}}$)} & \makecell{Storage Footprint} \\
        \midrule
    \multicolumn{7}{l}{\textbf{StaticIR}} \\
    \midrule
    
    $\text{Spider}_\text{ DE}$ & - & 19.65\% & - & 9.0e+10 & 18.9h & \textbf{24.48ms} / 26m & 173.8G \\
    $\text{Contriever}_\text{ DE}$ & - & 16.10\% & - & 9.0e+10 & 18.9h & 212.4ms\tnote{\textdagger} / 9.8m & 88.8G \\
    \hdashline[1pt/2pt]
    $\text{SEAL}_\text{ GR}$ & - & 34.95\% & - & \textbf{4.3e+10} & \textbf{2.7h} & 545.9ms / \textbf{1m 5s} & \textbf{34.5G} \\
    $\text{MINDER}_\text{ GR}$ & - & \textbf{37.90\%} & - & \textbf{4.3e+10} & \textbf{2.7h} & 424.6ms / \textbf{1m 5s} & \textbf{34.5G} \\
    \midrule
    \multicolumn{7}{l}{\textbf{Indexing-based Update}} \\
    \midrule
    $\text{Spider}_\text{ DE}$ & 24.82\% & 15.60\% & 34.03\% & 1.0e+11 & 20.4h & \textbf{24.84ms} / 28m & 196.8G \\
    $\text{Contriever}_\text{ DE}$ & 19.66\% & 13.75\% & 28.53\% & 1.0e+11 & 20.4h & 228.8ms\textsuperscript{\textdagger} / 10.5m & 99.8G \\
    \hdashline[1pt/2pt]
    $\text{SEAL}_\text{ GR}$ & 33.05\% & 32.75\% & 33.50\% & \textbf{4.3e+10} & \textbf{3.1h} & 612.2ms / \textbf{1m 26s} & \textbf{37.5G} \\
    $\text{MINDER}_\text{ GR}$ & \textbf{38.47\%} & \textbf{37.65\%} & \textbf{39.70\%} & \textbf{4.3e+10} & \textbf{3.1h} & 485.4ms / \textbf{1m 26s} & \textbf{37.5G} \\
    \midrule
    \multicolumn{7}{l}{\textbf{Training-based Update}} \\
    \midrule
    $\text{Spider}_\text{ DE}$ & 36.99\% & 21.75\% & \textbf{52.23\%} & 1.0e+11 & 20.4h & \textbf{24.84ms} / 28m & 196.8G \\
    $\text{Contriever}_\text{ DE}$ & 23.85\% & 8.20\% & 39.50\% & 1.0e+11 & 20.4h & 228.8m\textsuperscript{\textdagger} / 10.5m & 99.8G \\
    \hdashline[1pt/2pt]
    $\text{SEAL}_\text{ GR}$ & 41.01\% & 38.25\% & 43.77\% & \textbf{4.3e+10} & \textbf{3.1h} & 612.2ms / \textbf{1m 26s} & \textbf{37.5G}\\
    $\text{MINDER}_\text{ GR}$ & \textbf{41.54\%} & \textbf{38.85\%} & 44.23\% & \textbf{4.3e+10} & \textbf{3.1h} & 485.4ms / \textbf{1m 26s} & \textbf{37.5G}\\
    \bottomrule
    \end{tabular}
    }
      \begin{tablenotes}   
        %\item[\textdagger] We employ LoRA during the continual pretraining and apply it to DE for the next revision.
        \item[\textdagger] For Contriever, $T_{\textit{online}}$ is measured using faiss-cpu.
      \end{tablenotes}
\caption{Results of DynamicIR. Our experiments are divided into 3 setups, (1) StaticIR, (2) Indexing-based Updates, and (3) Training-based Updates. For each setups, we assess the performance on $Q_{\textit{total}}$, $Q_{\textit{initial}}$, and $Q_{\textit{new}}$, and efficiency which is evaluated using 4 metrics. We highlight the best scores in \textbf{bold} for each setup. 
For Inference Latency, $T_{\textit{online}}$ indicates the time required for query embedding and search, and $T_{\textit{offline}}$ indicates the time required for loading the indexed corpus. Additionally, the zero-shot performance for all models is provided in Appendix \ref{tabs:zeroshot}.}

%Specifically, for Inference Latency, we highlight in \textbf{bold} the time required query embeddings and search on the \textbf{left} and in \underline{underline} the time required for loading the indexed corpus on the \textbf{right}.
%The results of hit@5 performance and efficiency are detailed in Section \ref{} and \ref{}, respectively. 
\label{table: score}
%\stepcounter{mpFootnoteValueSaver}%
    %\footnotetext[\value{mpFootnoteValueSaver}]{%
      %{We employ LoRA during the continuous pretraining of a new corpus for the fully parametric model GR. The next revision will also involve applying LoRA for the pretraining of DE.}.}%
      \end{threeparttable}
\end{table*}



%\footnote{We employ LoRA during the continuous pretraining of a new corpus for the fully parametric model GR. The next revision will also involve applying LoRA for the pretraining of DE.}

==> tabs/static_results.tex <==
\begin{table*}[t!]
\centering
\fontsize{7.6}{13}\selectfont
    \begin{tabular}{ccccc}
        \toprule
             & \multicolumn{1}{c}{Performance $(hit@5)$} & \multicolumn{3}{c}{Efficiency} \\
                %\cmidrule(lr){2-4} \cmidrule(lr){5-8}  
             Evaluation & Base Corpus & Index Time & Infer Flops & Memory \\
        \midrule
    \multicolumn{1}{l}{\textbf{Dual Encoder}} \\
    \midrule
    Spider-$static$ & 19.65\% & - & - & 170G+3.8G \\
    Contriever-$static$ & 16.10\% & - & - & 170G+3.8G \\
    \midrule
    \multicolumn{1}{l}{\textbf{Generative Retrieval}} \\
    \midrule
    SEAL-$static$ & 34.95\% & 2.7H & - & 29G+5.5G \\
    MINDER-$static$ & 37.90\% & 2.7H & - & 29G+5.5G \\
    \bottomrule
    \end{tabular}
\caption{StaticIR}
\label{table: score}
\end{table*}

\label{tabs:static_results}

==> tabs/test.tex <==
\begin{table}
\centering
\label{t4}
\begin{tabular}{c|cc|cc}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{column1} & \multicolumn{2}{c}{column2} \\
\cline{2-5}
      & Fully-connected Layer  & Attention Layer & \\
\hline
  & - & - & - & - \\
 row2 & - & - & - & - \\
 row3 & - & - & - & - \\
\hline
\hline
\end{tabular}
\end{table}

==> tabs/train_update.tex <==
\begin{table*}[t!]
\centering
\fontsize{7.5}{13}\selectfont
    \begin{tabular}{ccccccccc}
        \toprule
             & \multicolumn{3}{c}{Performance $(hit@5)$} & \multicolumn{4}{c}{Efficiency} \\
                %\cmidrule(lr){2-4} \cmidrule(lr){5-8}  
             Evaluation & Total & Base & Update & TP & Flops & indexing & Inferece & Memory \\
        \midrule
    \multicolumn{8}{l}{\textbf{Dual Encoder}} \\
    \midrule
    Spider-$static$ & - & 18.2\% & - & 340M(3.8G) & - & - & - & 170G \\
    Contriever-$static$ & - & - & - & 340M(3.8G) & - & - & - & -\\
    \hdashline[1.5pt / 1.5pt]
    Spider-$update$ & 37.80\% (38.86\%) & 29.75\% (30.65\%) & 49.87\% (51.17\%) & 340M & - & - & - & 193G \\
    Contriever-$update$ & - & - & - & 340M & - & - & - & -\\
    \midrule
    \multicolumn{8}{l}{\textbf{Generative Retrieval}} \\
    \midrule
    SEAL-$static$ & - & 34.95\% & - & 406M(5.5G) & - & - & - & 29G\\
    MINDER-$static$ & - & 37.90\% & - & 406M(5.5G) & - & - & - & 29G\\
    \hdashline[1.5pt / 1.5pt]
    SEAL-$update$ & 40.46\% & 38.25\% & 43.77\% & 3.1M & - & - & - & 32G\\
    MINDER-$update$ & 41.00\% & 38.85\% & 44.23\% & 3.1M & - & - & - & 32G\\
    \bottomrule
    \end{tabular}
\caption
     {Advanced Update with Continual Pretraining}
\label{table: score}
\end{table*}
